$\clubsuit$ CLOVER $\clubsuit$: Probabilistic Forecasting with Coherent Learning Objective Reparameterization

Obtaining accurate probabilistic forecasts is an operational challenge in many applications, such as energy management, climate forecasting, supply chain planning, and resource allocation. Many of these applications present a natural hierarchical structure over the forecasted quantities; and forecasting systems that adhere to this hierarchical structure are said to be coherent. Furthermore, operational planning benefits from the accuracy at all levels of the aggregation hierarchy. However, building accurate and coherent forecasting systems is challenging: classic multivariate time series tools and neural network methods are still being adapted for this purpose. In this paper, we augment an MQForecaster neural network architecture with a modified multivariate Gaussian factor model that achieves coherence by construction. The factor model samples can be differentiated with respect to the model parameters, allowing optimization on arbitrary differentiable learning objectives that align with the forecasting system's goals, including quantile loss and the scaled Continuous Ranked Probability Score (CRPS). We call our method the Coherent Learning Objective Reparametrization Neural Network (CLOVER). In comparison to state-of-the-art coherent forecasting methods, CLOVER achieves significant improvements in scaled CRPS forecast accuracy, with average gains of 15%, as measured on six publicly-available datasets.

==> figures/factor_plot.tex <==
\begin{figure*}[ht]
\begin{subfigure}[b]{.28\textwidth}
    \centering
    \includegraphics[width=.9\columnwidth]{figures/Hist_concentration_gamma_favorita.png}
    \caption{Gamma factor concentrations}
    \label{subfig:hist_gamma_concentration}
\end{subfigure}
\begin{subfigure}[b]{.28\textwidth}
    \centering
    \includegraphics[width=.9\columnwidth]{figures/Hist_rate_gamma_favorita.png}
    \caption{Gamma factor rates}
    \label{subfig:hist_gamma_rate}
\end{subfigure}
\begin{subfigure}[b]{.4\textwidth}
    \centering
    \includegraphics[width=.9\columnwidth]{figures/Loadings_favorita.png}
    \caption{Loadings}
    \label{subfig:loadings}
\end{subfigure}
\caption{Analysis of factors and loadings. We show histograms of the learned factors for a given FCD, at lead time 0 in the left figures~\ref{subfig:hist_gamma_concentration}, \ref{subfig:hist_gamma_rate}. We show the loadings of each base-level region onto the learned factors in~\ref{subfig:loadings}. We see that the loadings have a banded structure. This is a placeholder plot to be improved.\ruijun{To fix caption}
} 
\label{fig:factors}
\end{figure*}

==> figures/n_factor_plot.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=.45\textwidth]{figures/n_factor_plot.png}
    \caption{Performance of our model for different numbers of factors based on one run with the same random seed. We provide overall normalized CRPS on \texttt{Traffic} for a model with Gamma factors and Clipped Normal base distributions. We also fit a 3-degree polynomial function to the results. 
    \vspace{-1\baselineskip}} 
\label{fig:n_factor_plot}
\end{figure}

==> tables/crps_full_all_baselines.tex <==
\input{nonmath_commands}

\begin{table*}[t] %[ht]
\small
\tabcolsep=0.11cm
\begin{tabular}{@{}l|l|l|lllllll@{}}
\toprule[1.5pt]
Dataset  &Metric& Level & Ours & DPMN-GroupBU        & DPMN-NaiveBU        & HierE2E     & ARIMA-MinT-Boot  & ARIMA-Normality & ARIMA-PermBU     \\ \midrule
\TourismL &CRPS& Overall &   $\mathbf{0.1101\pm 0.0009}$                    & $0.1249 \pm 0.0020$  & $0.1274 \pm 0.0028$           & $0.1456 \pm 0.0061$      &                             $0.1317\pm0.0008$  \\ 

  && Level 1 &   $0.0349\pm 0.0028$    & $0.0431 \pm 0.0042$  & $0.0514 \pm 0.0030$           & $0.0721 \pm 0.0095$      &$\mathbf{0.0277\pm0.0011}$                                    \\ 
  && Level 2 &   $\mathbf{0.0601\pm 0.0021}$                 & $0.0637 \pm 0.0032$  & $0.0705 \pm 0.0026$           & $0.0943 \pm 0.0059$   & $0.0628\pm0.0010$                                          \\ 
 && Level 3 &   $\mathbf {0.0959\pm 0.0027}$                 & $0.1084 \pm 0.0033$           & $0.1068 \pm 0.0019$  & $0.1280 \pm 0.0077$                     &$0.1150\pm0.0008$    \\ 
 && Level 4 &   $\mathbf{0.1372\pm 0.0022}$                 & $0.1554 \pm 0.0025$           & $0.1507 \pm 0.0014$  & $0.1682 \pm 0.0083$                                  &$0.1688\pm0.0007$   \\ 
 && Level 5 &   $\mathbf{0.0552\pm 0.0016}$                 &  $0.0700 \pm 0.0038$  & $0.0907 \pm 0.0061$           & $0.0992 \pm 0.0133$  &$0.0750\pm0.0014$                                \\ 
  && Level 6 &   $\mathbf{0.1000\pm 0.0009}$                 & $0.1070 \pm 0.0023$  & $0.1175 \pm 0.0047$           & $0.1361 \pm 0.0069$                            &$0.1221\pm 0.0014$      \\ 
  && Level 7 &   $\mathbf{0.1652\pm 0.0008}$                 & $0.1887 \pm 0.0032$           & $0.1836 \pm 0.0038$  & $0.1996 \pm 0.0072$    &$0.1976\pm0.0010$                            \\ 
 && Level 8 &   $\mathbf{0.2321\pm 0.0036}$                 & $0.2629 \pm 0.0034$           & $0.2481 \pm 0.0026$  & $0.2670 \pm 0.0073$ &$0.2841\pm0.0008$    \\ \midrule
 &RelMSE& Overall  &$\mathbf{0.0601\pm 0.0019}$  &$0.1113 \pm 0.0158$ & $0.2680 \pm 0.0748$ &$0.2058\pm0.0443$& 0.1075\\ \midrule[1pt]
\Favorita&CRPS& Overall &  $\mathbf{ 0.3080\pm 0.0201}$      &  $0.4020 \pm 0.0182$ & $0.5301 \pm 0.0120$            & $0.5099 \pm 0.1080$                 & $0.3968\pm0.0007$ \\ 
&& Country &  $\mathbf{0.2116\pm 0.0117}$      & $0.2760 \pm 0.0149$          & $0.4166 \pm 0.0195$           & $0.3521 \pm 0.1526$  & $0.2652\pm0.0005$       \\ 
&& State &  $\mathbf {0.2910\pm 0.0205}$      & $0.3865 \pm 0.0207$         & $0.5128 \pm 0.0108$           & $0.4860 \pm 0.1120$ & $0.3782\pm0.0006$ \\ 
&& City &  $\mathbf {0.3095\pm 0.0205}$      & $0.4068 \pm 0.0206$ & $0.5317 \pm 0.0115$            & $0.5293 \pm 0.1046$   & $0.4028\pm0.0008$         \\ 
&& Store &  $\mathbf {0.4201\pm 0.0162}$      &  $0.5387 \pm 0.0253$ & $0.6594 \pm 0.0150$         & $0.6723 \pm 0.0630$  & $0.5410\pm0.0010$   \\ \midrule
 &RelMSE & Overall & $\mathbf{0.5381\pm 0.0368}$    & $0.7563 \pm 0.0713$ &$0.9533 \pm 0.0201$ & $1.082\pm0.5473$ & $1.1270$  \\ \midrule[1pt]
\Traffic  &CRPS&Overall & $\mathbf{0.0181 \pm 0.0028 }$ &$0.0907 \pm 0.0024$           & $0.0704 \pm 0.0014$           & $0.0309 \pm 0.0062$          &$0.0731\pm0.0050$         \\
  &&Level 1 & $0.0176 \pm 0.0030$ &$0.0397 \pm 0.0044$           & $\mathbf{0.0134 \pm 0.0022}$  & $0.0157 \pm 0.0327$   &$0.0452\pm0.0066$                        \\
  &&Level 2 &  $0.0176 \pm 0.0030$& $0.0537 \pm 0.0024$          & $0.0289 \pm 0.0017 $          & $\mathbf{0.0103 \pm 0.0099}$   &$0.0470\pm0.0057$       \\
 &&Level 3 &  $\mathbf{0.0176 \pm 0.0031}$ & $0.0538 \pm 0.0022$           & $0.0290 \pm 0.0011$           & $0.0160 \pm 0.0093$    &$0.0544\pm0.0042$            \\
 &&Level 4 &  $\mathbf{0.0195 \pm 0.0028}$ & $0.2155 \pm 0.0022$           & $0.2101 \pm 0.0008$           & $0.0881 \pm 0.0094$    & $0.1459\pm0.0047$     \\ \midrule
 &RelMSE & Overall & $0.0232\pm 0.0536$ & $0.1750 \pm 0.0099$ & $0.0168 \pm 0.0026$ &$\mathbf{0.0047\pm0.0054}$& $0.0624$ \\
\bottomrule[1.5pt]
\end{tabular}
\caption{Results of our empirical evaluation. We report the CRPS score for each dataset (smaller is better) at various hierarchical levels (a level with lower number represents a more aggregated level, more details discussed in Appendix \ref{sec:level_details}). Average accuracy and its interval are computed based on three independent runs. Our model improves on previous methods on all datasets at all levels but Level 1 of \Traffic. On \TourismL, our model improves on the previous state of the art by $\TourismLgains\%$. 
On the larger-scale \Favorita dataset, our model improves by $\Favoritagains\%$. On \Traffic, we improve the best result by $\Trafficgains\%$ overall. Our model performs notably better at the finest granularity; our model's performance is stable across levels, whereas the other models perform better at the aggregate levels than at the base level. We evaluate our mean forecasts by computing the RelMSE score at the overall level (summing the total squared error at all levels, and normalize it by that of naive forecasts). Note ARIMA-MinT-Boot produces deterministic mean forecasts across model runs. 
Our model achieves lower RelMSE than other models on two datasets: $\TourismLMSEgains\%$ improvement on \TourismL, $\FavoritaMSEgains\%$ on \Favorita, but reaches higher RelMSE on \Traffic, despite large gains in CRPS. 
%\vspace{-\baselineskip}
}
\label{tab:results_allbaselines}
\end{table*}


==> tables/distributions_comparison.tex <==

% \begin{table}[ht]\small
% \begin{tabular}{@{}lcccc@{}}
% \toprule
%                   & Gamma & Log-Normal & Truncated Normal & Clipped Normal \\ \midrule
% \texttt{Tourism-Large}  & $0.1169$  & $0.1961$     & $0.1143$         &   $\\mathbf0.1138$       \\ 
% \texttt{Favorita} &  $ $   &    $ $        &         $ $         & $0.3165$  \\
% \texttt{Traffic} & $0.0475 \pm 0.0084$      &  $0.5761 \pm 0.1711$       &  $\\mathbf0.0243 \pm 0.0038$            & $\\mathbf0.0202 \pm 0.0041$\\\bottomrule
% \end{tabular}
% \caption{Performance of our model for various choices of base distribution. We provide overall CRPS scores for factor models Gamma factor and base distributions being Gamma, Log-Normal, Truncated Normal and Clipped Normal base distributions. The Gamma and Truncated-Normal distributions performed similarly for \texttt{Tourism-Large}, whereas the Clipped Normal outperformed the alternatives for \texttt{Favorita}. {\color{red} Placeholder while waiting for final results.}
% \vspace{-2\baselineskip}
% }
% \label{tab:base_dists}

% \end{table}

%KDD version%

\begin{table}[t]
\begin{center}
	\begin{tabular}{@{}lccc@{}}
			\toprule
			& \texttt{Tourism-Large} & \texttt{Favorita} & \texttt{Traffic} \\ \midrule
			
			Gamma & $0.1174\pm0.0044$  &    $0.4817\pm0.2274 $    &       $0.0738\pm0.0629$           \\ 
			Log-Normal  &  $0.2245\pm 0.0905$    &     $0.5268\pm0.1211$    &             $1.0135\pm0.2967$    \\
			Trunc-Normal &$0.1123\pm 0.0038$        &    $0.3922\pm0.0695$   &  $0.0216\pm0.0033 $    \\
			Clipped Normal  &$\mathbf {0.1101\pm0.0009}$   & $\mathbf {0.3080\pm0.0201}$&$\mathbf{0.0181\pm0.0028}$\\ \midrule
			\bottomrule
		\end{tabular}
\caption{Performance of our model for various choices of base distribution, where results are based on three independent runs. We provide overall normalized CRPS for factor models with Gamma distributed factors and various base distributions.} 
\label{tab:base_dists}
\end{center}
\end{table}
% \hspace{-\baselineskip}
% %ICDM version%
% \begin{table}[ht]
% \revision{ \small
% 	\begin{tabular}{@{}lccc@{}}
% 			\toprule
% 			& \texttt{Tourism-Large} & \texttt{Favorita} & \texttt{Traffic} \\ \midrule
			
% 			Gamma & $0.117\pm0.004$  &    $0.482\pm0.227 $    &       $0.074\pm0.063$           \\ 
% 			Log-Normal  &  $0.225\pm 0.091$    &     $0.527\pm0.121$    &             $1.014\pm0.297$    \\
% 			Trunc-Normal &$0.112\pm 0.004$        &    $0.392\pm0.070$   &  $0.022\pm0.003 $    \\
% 			Clipped Normal  &$\mathbf {0.110\pm0.001}$   & $\mathbf {0.308\pm0.020}$&$\mathbf{0.018\pm0.003}$\\ \midrule
% 			\bottomrule
% 		\end{tabular}
% }
% \caption{Performance of our model for various choices of base distribution, \revision{where all results are based on three independent run.} We provide overall normalized CRPS for factor models Gamma factor and various base distributions. 
% }
% \label{tab:base_dists}
% \end{table}

==> tables/number_of_factors_analysis.tex <==

% \begin{table}[ht]\small
% \begin{tabular}{@{}lcccc@{}}
% \toprule
%                   & Gamma & Log-Normal & Truncated Normal & Clipped Normal \\ \midrule
% \texttt{Tourism-Large}  & $0.1169$  & $0.1961$     & $0.1143$         &   $\bf0.1138$       \\ 
% \texttt{Favorita} &  $ $   &    $ $        &         $ $         & $0.3165$  \\
% \texttt{Traffic} & $0.0475 \pm 0.0084$      &  $0.5761 \pm 0.1711$       &  $\bf0.0243 \pm 0.0038$            & $\bf0.0202 \pm 0.0041$\\\bottomrule
% \end{tabular}
% \caption{Performance of our model for various choices of base distribution. We provide overall CRPS scores for factor models Gamma factor and base distributions being Gamma, Log-Normal, Truncated Normal and Clipped Normal base distributions. The Gamma and Truncated-Normal distributions performed similarly for \texttt{Tourism-Large}, whereas the Clipped Normal outperformed the alternatives for \texttt{Favorita}. {\color{red} Placeholder while waiting for final results.}
% \vspace{-2\baselineskip}
% }
% \label{tab:base_dists}

% \end{table}

\begin{table}[ht]
\begin{tabular}{@{}lcccccc@{}}
\toprule
\# Factors                 & 1 & 2 & 3 & 4 & 5 & 10 \\ \midrule
CRPS & $0.3170$ & $0.3256$ & $0.32275$ & $0.3484$ & $0.3186$ & $\bf0.3101$\\ \midrule
\bottomrule
\end{tabular}
\caption{Performance of our model for different numbers of factors where results of 10 factor is based on three independent run, and other results are based on a single run. We provide overall normalized CRPS on \texttt{Favorita} for a model with Gamma factors and Clipped Normal base distributions. 
%\vspace{-2\baselineskip}
}
\label{tab:n_factors}

\end{table}

